Optimized Generic Feature Learning for Few-shot Classification across Domains

To learn models or features that generalize across tasks and domains is one of the grand goals of machine learning. In this paper, we propose to use cross-domain, cross-task data as validation objective for hyper-parameter optimization (HPO) to improve on this goal. Given a rich enough search space, optimization of hyper-parameters learn features that maximize validation performance and, due to the objective, generalize across tasks and domains. We demonstrate the effectiveness of this strategy on few-shot image classification within and across domains. The learned features outperform all previous few-shot and meta-learning approaches.

==> tables/cross_domain_compare.tex <==
\begin{tabular}{lccccc}
\hline 
\multicolumn{1}{l}{\bf Test source}  &  \multicolumn{1}{c}{\bf Proto-MAML}  &  \multicolumn{1}{c}{\bf BOHB-Linear}  &  \multicolumn{1}{c}{\bf BOHB-Cosine}  &  \multicolumn{1}{c}{\bf BOHB-X-Linear}  &  \multicolumn{1}{c}{\bf BOHB-X-Cosine} \\ \hline \\ 
Omniglot                    &   $63.00\pm1.35$              &   $64.09\pm1.36$              &   $67.57\pm1.21$              &   $65.14\pm1.33$              &   $68.08\pm1.20$            \\ 
Aircraft                    &   $55.31\pm0.96$              &   $57.36\pm1.04$              &   $54.12\pm0.90$              &   $54.02\pm1.05$              &   $55.76\pm0.93$            \\ 
Birds                       &   $66.87\pm1.04$              &   $67.68\pm1.08$              &   $70.69\pm0.90$              &   $67.27\pm1.02$              &   $68.12\pm0.98$            \\ 
Textures                    &   $67.75\pm0.78$              &   $70.38\pm0.91$              &   $68.34\pm0.76$              &   $69.27\pm0.85$              &   $68.50\pm0.68$            \\ 
QuickDraw                   &   $53.70\pm1.06$              &   $46.26\pm1.27$              &   $50.33\pm1.04$              &   $50.17\pm1.25$              &   $50.93\pm1.02$            \\ 
Fungi                       &   $37.97\pm1.11$              &   $33.82\pm1.03$              &   $41.38\pm1.12$              &   $34.78\pm1.11$              &   $41.16\pm1.09$            \\ 
VGG Flower                  &   $86.86\pm0.75$              &   $85.51\pm0.75$              &   $87.34\pm0.59$              &   $86.36\pm0.69$              &   $87.37\pm0.59$            \\ 
Traffic Sign                &   $51.19\pm1.11$              &   $55.17\pm1.33$              &   $51.80\pm1.04$              &   $54.17\pm1.32$              &   $55.06\pm1.04$            \\ 
MSCOCO                      &   $43.41\pm1.06$              &   $41.58\pm1.17$              &   $48.03\pm0.99$              &   $41.88\pm1.14$              &   $46.96\pm1.04$            \\ 
\hline 
Average (cross domain)      &   $58.45\pm1.02$              &   $57.98\pm1.10$              &   $59.96\pm0.95$              &   $58.12\pm1.08$              &   $\mathbf{60.22\pm0.95}$            \\ 
\end{tabular}

==> tables/cross_domain_linear.tex <==
\begin{tabular}{lcccccc}
\multicolumn{1}{c}{\bf Test source}  &  \multicolumn{1}{c}{\bf S1}  &  \multicolumn{1}{c}{\bf S2}  &  \multicolumn{1}{c}{\bf S3}  &  \multicolumn{1}{c}{\bf S4}  &  \multicolumn{1}{c}{\bf Dataset score}  &  \multicolumn{1}{c}{\bf BOHB-Linear} \\ \hline \\ 
Omniglot                    &   $62.98\pm1.38$              &   $-$                         &   $-$                         &   $67.30\pm1.28$              &   $65.14\pm1.33$              &   $64.09\pm1.36$            \\ 
Aircraft                    &   $-$                         &   $-$                         &   $54.02\pm1.05$              &   $-$                         &   $54.02\pm1.05$              &   $57.36\pm1.04$            \\ 
Birds                       &   $-$                         &   $67.27\pm1.02$              &   $-$                         &   $-$                         &   $67.27\pm1.02$              &   $67.68\pm1.08$            \\ 
Textures                    &   $-$                         &   $69.27\pm0.85$              &   $-$                         &   $-$                         &   $69.27\pm0.85$              &   $70.38\pm0.91$            \\ 
QuickDraw                   &   $-$                         &   $-$                         &   $50.17\pm1.25$              &   $-$                         &   $50.17\pm1.25$              &   $46.26\pm1.27$            \\ 
Fungi                       &   $-$                         &   $-$                         &   $-$                         &   $34.78\pm1.11$              &   $34.78\pm1.11$              &   $33.82\pm1.03$            \\ 
VGG Flower                  &   $86.36\pm0.69$              &   $-$                         &   $-$                         &   $-$                         &   $86.36\pm0.69$              &   $85.51\pm0.75$            \\ 
Traffic Sign                &   $55.46\pm1.35$              &   $54.33\pm1.28$              &   $51.33\pm1.31$              &   $55.55\pm1.32$              &   $54.17\pm1.32$              &   $55.17\pm1.33$            \\ 
MSCOCO                      &   $42.17\pm1.14$              &   $43.26\pm1.20$              &   $40.52\pm1.14$              &   $41.57\pm1.10$              &   $41.88\pm1.14$              &   $41.58\pm1.17$            \\ 
%Average score               &   $61.74\pm1.14$              &   $58.53\pm1.09$              &   $49.01\pm1.19$              &   $49.80\pm1.20$              &   $58.12\pm1.08$              &   $57.98\pm1.10$            \\ 
\hline 
Average score               &                 &            &                &                &   $58.12\pm1.08$              &   $57.98\pm1.10$            \\ 
\end{tabular}

==> tables/data_schedule.tex <==
\begin{tabular}{lllcccc}
\hline 
\textbf{Datasets}      & \\ 
\hline
\end{tabular}

==> tables/image_resolution_compare.tex <==
\begin{tabular}{lcc}
\hline 
\textbf{Model}  & \textbf{Resolution} & \textbf{Cross-domain acc.} \\ 
\hline 
ProtoMAML       & $126\times126$      & $58.45\pm1.02$ \\ 
BOHB-Linear     & $126\times126$      & $57.98\pm1.10$ \\
BOHB-Cosine     & $126\times126$      & $59.96\pm0.95$ \\
BOHB-Linear     & $224\times224$      & $?$ \\ 
BOHB-Cosine     & $224\times224$      & $\mathbf{61.91\pm0.95}$ \\ 
\hline 
\end{tabular}



==> tables/mini_imagenet_compare.tex <==
\begin{tabular}{lcc}
\hline 
\textbf{Model}                      & \textbf{1-shot} & \textbf{5-shot} \\ 
\hline 
Baseline~\cite{closerlook}          & $51.75\pm0.80$             & $74.27\pm0.63$ \\
Baseline++~\cite{closerlook}        & $51.87\pm0.77$             & $75.68\pm0.63$ \\
MatchingNet~\cite{closerlook}       & $52.91\pm0.88$             & $68.88\pm0.69$ \\
ProtoNet~\cite{closerlook}          & $54.16\pm0.82$             & $73.68\pm0.65$ \\
MAML~\cite{closerlook}              & $49.61\pm0.92$             & $65.72\pm0.77$ \\ 
RelationNet~\cite{closerlook}       & $52.48\pm0.86$             & $69.83\pm0.68$ \\
\hline 
BOHB-Linear                         & $54.55\pm0.80$             & $76.99\pm0.62$ \\
BOHB-Cosine                         & $\mathbf{59.64\pm0.77}$    & $\mathbf{78.29\pm0.59}$ \\
\hline 
\end{tabular}


==> tables/train_all.tex <==
\begin{tabular}{lccccc}
\multicolumn{1}{c}{\bf Test source}  &  \multicolumn{1}{c}{\bf Proto-MAML}  &  \multicolumn{1}{c}{\bf D1 val}  &  \multicolumn{1}{c}{\bf D2 val}  &  \multicolumn{1}{c}{\bf Schedule D1 val}  &  \multicolumn{1}{c}{\bf Schedule D2 val} \\ \hline \\ 
ILSVRC                      &   $47.85\pm0.00$              &   $40.04\pm1.05$              &   $39.37\pm1.02$              &   $40.79\pm1.09$              &   $43.01\pm1.11$            \\ 
\hline 
Omniglot                    &   $82.86\pm0.00$              &   $87.29\pm0.85$              &   $88.38\pm0.78$              &   $83.82\pm0.95$              &   $88.30\pm0.80$            \\ 
Aircraft                    &   $74.24\pm0.00$              &   $74.80\pm0.90$              &   $73.85\pm0.78$              &   $75.96\pm0.75$              &   $81.18\pm0.74$            \\ 
Birds                       &   $69.97\pm0.00$              &   $61.12\pm1.14$              &   $61.99\pm1.06$              &   $66.50\pm1.01$              &   $67.42\pm0.99$            \\ 
Textures                    &   $67.94\pm0.00$              &   $64.92\pm0.83$              &   $63.37\pm0.84$              &   $65.07\pm0.76$              &   $65.67\pm0.79$            \\ 
QuickDraw                   &   $66.57\pm0.00$              &   $72.80\pm0.90$              &   $72.81\pm0.88$              &   $65.58\pm0.93$              &   $70.49\pm0.92$            \\ 
Fungi                       &   $41.99\pm0.00$              &   $38.25\pm1.12$              &   $36.37\pm1.11$              &   $42.32\pm1.06$              &   $46.94\pm1.13$            \\ 
VGG Flower                  &   $88.45\pm0.00$              &   $82.50\pm0.83$              &   $81.67\pm0.86$              &   $83.85\pm0.81$              &   $85.07\pm0.74$            \\ 
\hline 
Traffic Signs               &   $52.32\pm0.00$              &   $51.36\pm1.34$              &   $50.47\pm1.25$              &   $52.22\pm1.26$              &   $54.06\pm1.26$            \\ 
MS-COCO                     &   $41.29\pm0.00$              &   $38.56\pm1.13$              &   $37.05\pm1.08$              &   $36.63\pm1.05$              &   $38.97\pm1.03$            \\ 
\hline 
\hline 
Score (D1)                      &   $47.85\pm0.00$              &   $40.04\pm1.05$              &   $39.37\pm1.02$              &   $40.79\pm1.09$              &   $43.01\pm1.11$            \\ 
Score (D2)                  &   $70.29\pm0.00$              &   $68.81\pm0.94$              &   $68.35\pm0.90$              &   $69.01\pm0.90$              &   $72.15\pm0.87$            \\ 
Score (D3)                  &   $46.80\pm0.00$              &   $44.96\pm1.23$              &   $43.76\pm1.17$              &   $44.42\pm1.16$              &   $46.52\pm1.15$            \\ 
\end{tabular}
